Large-scale randomized experiment reveals machine learning helps people learn and remember more effectively

Machine learning has typically focused on developing models and algorithms that would ultimately replace humans at tasks where intelligence is required. In this work, rather than replacing humans, we focus on unveiling the potential of machine learning to improve how people learn and remember factual material. To this end, we perform a large-scale randomized controlled trial with thousands of learners from a popular learning app in the area of mobility. After controlling for the length and frequency of study, we find that learners whose study sessions are optimized using machine learning remember the content over $\sim$67% longer than those whose study sessions are generated using two alternative heuristics. Our randomized controlled trial also reveals that the learners whose study sessions are optimized using machine learning are $\sim$50% more likely to return to the app within 4-7 days.

==> 060pseudocode.tex <==
\begin{algorithm}                    % enter the algorithm environment
  \caption{\textsc{Select} Find the probability of selection of an item for study for one user}
  \label{alg:select}
%  \setstretch{1.5}
  \begin{algorithmic}[1]
  \State \textbf{Input: } Set of items $\Jcal$, number of (un)successful recalls $n^{\cmark}_i(t)$ and $n^{\xmark}_i(t)$, initial difficulties $\{ n_i(0) \}$, last review times $\{ t_i \}$ and parameters $\alpha$, $\beta$ and $q$.
  \State \textbf{Output: } Probability of selection of each item $\mathbf{p}(t)$. 

  \State $\mathbf{p}(t) \leftarrow \mathbf{0}$
  \For {$i \in \Jcal$}
    \State $n_i(t) \leftarrow n_i(0) (1 - \alpha)^{n^{\cmark}_i(t)} (1 + \beta)^{n^{\xmark}_i(t)}$
    \State $m_i(t) \leftarrow \exp{ \left( -n_i(t) (t - t_i) \right) }$ \Comment Using exponential memory model
    \State $p_i(t) = \frac{1}{\sqrt{q}}(1 - m_i(t))$
  \EndFor

%  \State $\Pbar \leftarrow \sum_{i \in \Jcal} p_i

  \State \Return $\mathbf{p}(t)$

%   \State $F_0 \leftarrow $ \textbf{\textsc{Evaluate}}$(\Xcal_0)$
%
%       \For {$g \in [0, \dots, G - 1]$}
%           \State $U \leftarrow$ \textsc{SelTournamentCDC}$(\Xcal_g, F_g)$ \Comment{Select off-springs using tournaments~\cite{deb2002}}
%           \State $V \leftarrow \varnothing$
%
%           \State $Z_1 \leftarrow$ \textsc{RandomChoose}$(U, P / 2)$ \Comment Partition $U$ into 2 equal sets
%           \State $Z_2 \leftarrow Y \cap Z_1$
%
%           \For {$i \in [1, \dots, P / 2]$}
%               \State $o_1 \leftarrow $ \textsc{RandomChoose}$(Z_1, 1)$
%               \State $o_2 \leftarrow $ \textsc{RandomChoose}$(Z_2, 1)$
%
%               \State $Z_1 \leftarrow Z_1 \setminus \{ o_1 \}$
%               \State $Z_2 \leftarrow Z_2 \setminus \{ o_2 \}$
%
%               \If {\textsc{Random}$() < p_x$}
%                  \State $o_1, o_2 \leftarrow $ \textsc{Mate}$(o_1, o_2)$
%               \EndIf
%
%               \State $V \leftarrow V \cup \{ o_1, o_2 \}$
%           \EndFor
%
%           \State $\Xcal_{g + 1} \leftarrow \varnothing$
%           \For {$o \in V$}
%               \If {\textsc{Random}$() < p_m$}
%                   \State $o \leftarrow $ \textsc{Mutate}$(o)$ \Comment Random binary noise for each bit
%               \EndIf
%
%               \State $\Xcal_{g + 1} \leftarrow \Xcal_{g + 1} \cup \{ o \}$
%           \EndFor
%
%           \State $F_{g + 1} \leftarrow $ \textbf{\textsc{Evaluate}}$(\Xcal_{g + 1})$
%     \EndFor
%
%     \State \Return \textsc{Pareto}$\left( \bigcup_{g \in [0, \dots, G]} \left\{ \Xcal_g \right\} \right)$
  \end{algorithmic}
\end{algorithm}


